On Parameterized Complexity of Liquid Democracy

In liquid democracy, each voter either votes herself or delegates her vote to some other voter. This gives rise to what is called a delegation graph. To decide the voters who eventually votes along with the subset of voters whose votes they give, we need to resolve the cycles in the delegation graph. This gives rise to the Resolve Delegation problem where we need to find an acyclic sub-graph of the delegation graph such that the number of voters whose votes they give is bounded above by some integer {\lambda}. Putting a cap on the number of voters whose votes a voter gives enable the system designer restrict the power of any individual voter. The Resolve Delegation problem is already known to be NP-hard. In this paper we study the parameterized complexity of this problem. We show that Resolve Delegation is para-NP-hard with respect to parameters {\lambda}, number of sink nodes and the maximum degree of the delegation graph. We also show that Resolve Delegation is W[1]-hard even with respect to the treewidth of the delegation graph. We complement our negative results by exhibiting FPT algorithms with respect to some other parameters. We finally show that a related problem, which we call Resolve Fractional Delegation, is polynomial time solvable.

==> a1.tex <==
\section{Omitted Proofs}
\begin{corollary}\label{cor:lambda_D_bipartite}
Given that the input graph is both bipartite and directed acyclic graph, the \rd problem is \NPC even if we have $\lambda=3$ and both the out-degree and in-degree of every vertex is at most $3$ which concludes that \rd is \PNPH with respect to the parameter $(\lambda,\Delta)$.
\end{corollary}
\begin{proof}
The proof follows as the resulting graph \GG from reduction of \tsat instance in Theorem \ref{thm:lambda_D} is bipartite and directed acyclic graph (DAG).
\end{proof}
\begin{corollary}\label{cor:bip}
\rd is W[1]-hard when parameterized by the treewidth even when the input graph is both Bipartite and Directed Acyclic Graph. 
\end{corollary}
\begin{proof}
In the instance of \rd created in Theorem \ref{thm:treewidth}, graph $\mathcal{H}$ is Bipartite as there is no odd cycle in the underlying undirected graph.  Also graph $\mathcal{H}$ is Directed Acyclic Graph (DAG) 
\end{proof}
\begin{observation}\label{obs:lambda_t}
	There is a kernel for \rd consisting of at most $\lambda t$ vertices. In particular, there is an \FPT algorithm for the \rd problem parameterized by $(\lambda,t)$.
\end{observation}
\begin{proof}
	If the number $n$ of vertices in the input graph is more than $\lambda t$, then the instance is clearly a \NO instance. Hence, we have $n\le\lambda t$.
\end{proof}
%% bipartitie


%\begin{theorem}\label{thm:t_bipartites}
%	Given that the input instance is bipartite graph, the \rd problem is \NPC even if we have only $2$ sink vertices. Thus \rd is \PNPH with respect to the parameter $t$.
%\end{theorem}


%\begin{proof}
%Intuitively we follow similar reduction technique as in \ref{thm:t} with different weights on the additional subgraphs included during reduction.

	%We reduce \tvdp to our problem as follows : Let $(\GG=(\VV,\EE),s_1,t_1,s_2,t_2)$ be an arbitrary instance of \tvdp. We first consider an equivalent instance of \tvdp. Let $\GG^{b}$ be the instance constructed from \GG as follows : 
	%\begin{align*}
%		\VV^{b} &= \{b_v: v\in\VV\} \cup \VV_{e} \text{ where}\\
%		& \VV_{e}=\{b_{u,v} : (u,v) \in\EE\}\\
%		\EE^{b} &= \{(b_u, b_{u,v}), (b_{u,v}, b_{v}) : (u,v)\in\EE\}
%	\end{align*}
%Clearly $\GG^{b}$ has twice the number of edges in \GG.
 %Note that $\VV^b$ can be partitioned into $ \{b_v: v\in\VV\}$ and $\VV_e$. Also $ \{b_v: v\in\VV\}$ and $\VV_e$ are independent sets. So $\GG^{b}$ is a bipartite graph. 
%The claim follows by ensuring that there all cycles in the graph are of even path length. Since every edge in \GG is replaced by two edges in $\GG^{b}$, we can claim that every path in \GG (including cycles) has doubled in path length in $\GG^{b}$ which proves the claim. 
%It can also be seen that the two instances are still equivalent.\\
%We now construct the the instance $(\GG^\pr=(\VV^\pr,\EE^\pr),\lambda)$ as shown below:
%	\begin{align*}
%		\VV^\pr &= \{a_v: v\in\VV^{b}\} \cup \DD_1 \cup \DD_1^\pr\cup \DD_2\cup \DD_2^\pr \text{ where}\\
%		& |\DD_1|=|\DD_2^\pr|=10n_{b}, |\DD_1^\pr|=|\DD_2|=5n_{b} \quad \text{where} \quad n_{b}=|\VV^{b}|\\
%		\EE^\pr &= \{(a_u, a_v): (u,v)\in\EE^{b}\} \cup \FF 
%	\end{align*}
%		We now describe the edges in \FF. Each $\DD_1, \DD_1^\pr, \DD_2,$ and $\DD_2^\pr$ induces a path in $\GG^\pr$. The end vertices of the path induced on $\DD_1$ and $\DD_2$ be respectively $d_1$ and $d_2$. The start vertices of the path induced on $\DD_1^\pr$ and $\DD_2^\pr$ be respectively $d_1^\pr$ and $d_2^\pr$. The end vertices of the path induced on $\DD_1^\pr$ and $\DD_2^\pr$ be respectively $t_1^\pr$ and $t_2^\pr$. The set \FF also contains the edges in $\{(d_1,a_{s_1}), (d_2,a_{s_2}), (a_{t_1},d_1^\pr), (a_{t_2},d_2^\pr)\}$. This finishes the description of \FF and thus the description of $\GG^\pr$. We observe that $\GG^\pr$ has exactly $2$ sink vertices, namely $t_1^\pr$ and $t_2^\pr$. Finally we define $\lambda=17n_{b}$.
%We now prove that the instances \tvdp on the graph $\GG^{b}$ and \rd on graph $\GG'$ are equivalent.

%	In one direction, let us assume that the instance of \tvdp on the graph $\GG^{b}$ is a \YES instance. Let $\PP_i$ be a path from $s_i$ to $t_i$ in \GG such that $\PP_1$ and $\PP_2$ are vertex disjoint. Let \HH be a spanning sub-graph of $\GG^{b}$ which is connected (that is, if we disregard the direction of edges, then every vertex in reachable from every other vertex) and contains the paths $\PP_1$ and $\PP_2$. We define $\HH^\pr=(\VV^\pr,\EE^\prr)\subseteq\GG^\pr$ where 
%	$$\EE^\prr=\{(a_u, a_v): (u,v)\in\EE[\HH]\} \cup \FF$$

%	We observe that the out degree of every vertex is exactly $1$ in $\HH^\pr$ except the sink vertices in $\GG^\pr$ (which are $t_1^\pr$ and $t_2^\pr$). Also since \HH contains the path $\PP_i$, every vertex in $\DD_i$ has a path to $t_i^\pr$ for $i\in[2]$. Of course, every vertex in $\DD_i^\pr$ has a path to $t_i^\pr$ for $i\in[2]$. Hence the number of vertices which has a path to $t_i$ in $\HH^\pr$ is at most $16n_{b}$ which is less than \lambda. Hence the \rd instance is a \YES instance.
	
%	In the other direction, let us assume that the \rd instance is a \YES instance. Let $\HH^\pr=(\VV^\pr,\EE^\prr)\subseteq\GG^\pr$ be a spanning sub-graph of $\GG^\pr$ such that (i) the out degree of every vertex which is not a sink is exactly $1$, (ii) there are at most $\lambda$ vertices in $\HH^\pr$ which has a path to $t_i^\pr$ for $i\in[2]$. We observe that, for $i\in[2]$, $a_{s_i}$ must have a path $\PP_i^\pr$ to $a_{t_i}$ in $\HH^\pr$ otherwise there are at most $10n$ vertices have path to $t_i^\pr$ and thus at least $20n_{b}$ vertices have path to $t_{3-i}^\pr$ in $\HH^\pr$ which is a contradiction (since $\lambda=17n_{b}$). We define a spanning sub-graph $\HH\subseteq\GG^{b}$ as $\EE[\HH]=\{(u,v):(a_u,a_v)\in\EE^\prr\}$. Since, for $i\in[2]$, we have a path $\PP_i^\pr$ from $a_{s_i}$ to $a_{t_i}$ in $\HH^\pr$ and the out-degree of every vertex except $t_1^\pr$ and $t_2^\pr$ is $1$, the paths $\PP_1^\pr$ and $\PP_2^\pr$ are vertex disjoint. We define path $\PP_i=\{(u,v): (a_u,a_v)\in\PP_i^\pr\}$ in $\GG^{b}$ for $i\in[2]$. Since $\PP_1^\pr$ and $\PP_2^\pr$ are vertex disjoint, it follows that $\PP_1$ and $\PP_2$ are also vertex disjoint. Thus the \rd instance is a \YES instance.\\
%	To complete the result, we are left to prove that the resulting graph $\GG^\pr$ is a bipartite graph. The claim follows as $\GG^\pr$ is a union of $\GG^{b}$ which is a bipartite graph and four paths. Additional edges introduces between these also maintain the bipartite property. Thus the equivalence of the two instances $\GG$ and $\GG^{b}$ concludes that the problem \tvdp reduces in polynomial time to bipartite graph - \rd. This concludes the proof.
%\end{proof}
%% bipartite 

